String Solving with Stabilization and Transducers (Technical Report)

We generalize an efficient automata-based approach to string constraint solving, the stabilization-based method behind the solver Z3-Noodler, to support relational constraints represented by finite-state transducers (useful, for example, for modeling replaceAll constraints). We focus on an efficient treatment of length constraints by reducing the need for expensive concatenation elimination, which is a major bottleneck in automata-based string solving. We also propose powerful heuristics that significantly improve performance in practice. Implemented on top of Z3-Noodler, our method vastly outperforms existing solvers on benchmarks with relational constraints. It solves more instances and runs orders of magnitude faster.

==> macromove.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% a transition as an arrow interrupted by a symbol in a bracket
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{trimclip}

\makeatletter
\DeclareRobustCommand{\shortto}{%
  \mathrel{\mathpalette\short@to\relax}%
}

\DeclareRobustCommand{\shortminus}{%
  \mathrel{\mathpalette\short@minus\relax}%
}

\newcommand{\short@to}[2]{%
  \mkern2mu
  \clipbox{{.5\width} 0 0 0}{$\m@th#1\vphantom{+}{\rightarrow}$}%
}

\newcommand{\short@minus}[2]{%
  \mkern2mu
  \clipbox{{.5\width} 0 0 0}{$\m@th#1\vphantom{+}{-}$}%
}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%variants of the transition arrow
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%scriptstyle
%-------------------------------
%-[bla]->
%\newcommand{\labeledto}[1]{{{\shortminus}\hspace{-1.6pt}\raisebox{0.16ex}{$\scriptstyle[ #1\hspace{-0.28pt}]$}\hspace{-2.2pt}{\shortto}}}
%-<bla>->
%\newcommand{\labeledto}[1]{{{\shortminus}\hspace{-2pt}\raisebox{0.16ex}{$\scriptstyle\langle #1\hspace{-0.28pt}\rangle$}\hspace{-2.2pt}{\shortto}}}
%-{bla}->
%\newcommand{\labeledto}[1]{{{\shortminus}\hspace{-2pt}\raisebox{0.16ex}{$\scriptstyle\{ #1\hspace{-0.28pt}\}$}\hspace{-2.2pt}{\shortto}}}
%-(bla)->
%\newcommand{\labeledto}[1]{{{\shortminus}\hspace{-1.0pt}\raisebox{0.16ex}{$\scriptstyle( #1\hspace{-0.28pt})$}\hspace{-1.6pt}{\shortto}}}
%-------------------------------
%small
%-------------------------------
%-[bla]->
%\newcommand{\labeledto}[1]{{{\shortminus}\hspace{-1.6pt}\raisebox{0.16ex}{$\scriptstyle[ #1\hspace{-0.28pt}]$}\hspace{-2.2pt}{\shortto}}}
%-<bla>->
%\newcommand{\labeledto}[1]{{{\shortminus}\hspace{-2pt}\raisebox{0.16ex}{$\scriptstyle\langle #1\hspace{-0.28pt}\rangle$}\hspace{-2.2pt}{\shortto}}}
%-{bla}->
\newcommand{\labeledto}[1]{{{\shortminus}\hspace{-2pt}\raisebox{0.16ex}{$\scriptstyle\{ #1\hspace{-0.28pt}\}$}\hspace{-2.2pt}{\shortto}}}
\newcommand{\labeledtotrans}[1]{{{\shortminus}\hspace{-2pt}\raisebox{0.16ex}{$\scriptstyle\{ #1\hspace{-0.28pt}\}$}\hspace{-2.2pt}{\shortto}^*}}
%-(bla)->
%\newcommand{\labeledto}[1]{\raisebox{-0.2pt}{\scalebox{1.2}{\ensuremath{{\shortminus}\hspace{-1.0pt}\raisebox{0.16ex}{$\scriptstyle(#1\hspace{-0.28pt})$}\hspace{-1.75pt}{\shortto}}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%automata arrow in superscript and subscritp script, so far only the -{bla}->
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\scriptlabeledto}[1]{{{\shortminus}\hspace{-1.0pt}\raisebox{0.12ex}{$\scriptscriptstyle\{ #1\hspace{-0.28pt}\}$}\hspace{-1.6pt}{\shortto}}}

% \def\moveStrange(#1,#2,#3){%somewhat shorter syntax 
% \mathchoice
% {#1\,\labeledto{#2}\,#3}
% {#1\labeledto{#2}#3}
% {#1\scriptlabeledto{#2}#3}
% {#1\scriptlabeledto{#2}#3}
% }
\newcommand\move[3]{%standard LaTex syntax where each parameter is put in {}
\mathchoice
{#1\,\labeledto{#2}\,#3}
{#1\labeledto{#2}#3}
{#1\scriptlabeledto{#2}#3}
{#1\scriptlabeledto{#2}#3}
}


==> macros.tex <==

\makeatletter
\newcommand*{\relrelbarsep}{.386ex}
\newcommand*{\relrelbar}{%
  \mathrel{%
    \mathpalette\@relrelbar\relrelbarsep
  }%
}
\newcommand*{\@relrelbar}[2]{%
  \raise#2\hbox to 0pt{$\m@th#1\relbar$\hss}%
  \lower#2\hbox{$\m@th#1\relbar$}%
}
\providecommand*{\rightrightarrowsfill@}{%
  \arrowfill@\relrelbar\relrelbar\rightrightarrows
}
\providecommand*{\leftleftarrowsfill@}{%
  \arrowfill@\leftleftarrows\relrelbar\relrelbar
}
\providecommand*{\xrightrightarrows}[2][]{%
  \ext@arrow 0359\rightrightarrowsfill@{#1}{#2}%
}
\providecommand*{\xleftleftarrows}[2][]{%
  \ext@arrow 3095\leftleftarrowsfill@{#1}{#2}%
}
\makeatother

% Arrow over a horizontal line (like an equals sign but with an arrow above)
% Usage: \arroweq or \arroweq[<width>] to specify the width of the underline
% Simpler, robust implementation: arrow over a horizontal rule using \overset.
% Usage: \arroweq or \arroweq[<width>] to specify the width of the underline
% simpler stacking using \overset to avoid alignment groups and missing-$ errors
% draw arrow slightly shorter than the rule so the arrow head doesn't overshoot
\newcommand{\arroweq}[1][2mm]{%
	% Draw an underline with a thin arrow very close above it (precise control via TikZ)
	\begingroup
		% total underline width
		\dimen0=#1\relax
		\ifdim\dimen0<0pt \dimen0=0pt\fi
		% vertical gap between underline and arrow baseline (smaller -> closer)
		\dimen2=0.5ex\relax
		% shorten arrow so head doesn't overshoot the underline
		\dimen4=0.0ex\relax
		\dimen6=\dimen0\relax
		\advance\dimen6 by -\dimen4\relax
		\ifdim\dimen6<0pt \dimen6=0pt\fi
		\ensuremath{\mathrel{%
			\begin{tikzpicture}[
				baseline={(base.south)},
				x=1pt, y=1pt,
				reset cm,
				transform shape=false,
				every picture/.style={},
				every path/.style={},
				every node/.style={},
				>=stealth',
				draw=black
			]
				\coordinate (base) at (0,0);
				% underline (keep standard thin rule thickness)
				\draw[line width=0.5pt] (0pt,0pt) -- (\the\dimen0,0pt);
				% arrow just above, thinner line
				\draw[->, line width=0.5pt] (0pt,\the\dimen2) -- (\the\dimen6,\the\dimen2);
			\end{tikzpicture}%
		}}%
	\endgroup
}

\newcommand\xqed[1]{%
  \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
  \quad\hbox{#1}}
\newcommand\sectionEndSymbol{\xqed{$\blacksquare$}}



%\newcommand{\tinytodo}[2][]
%{\todo[caption={#2}, size=\tiny, linecolor=black!70!white, backgroundcolor=white,
%		bordercolor=black!70!white, textcolor=black!70!white, size=\tiny#1]{\renewcommand{\baselinestretch}{0.5}\selectfont#2\par}}
%\newcommand{\lh}[1]{\textcolor{red!70}{\ifmmode \text{[LH: #1]}\else [LH: #1] \fi}}
%\newcommand{\js}[1]{\textcolor{purple}{\ifmmode \text{[JS: #1]}\else [JS: #1] \fi}}
%%\newcommand{\vh}[1]{\textcolor{green!70!black}{\ifmmode \text{[VH: #1]}\else [VH: #1] \fi}}
%\newcommand{\yfc}[1]{\textcolor{blue!70!black}{\ifmmode \text{[YFC: #1]}\else [YFC: #1] \fi}}
%% \newcommand{\dch}[1]{\textcolor{orange}{\ifmmode \text{[DCH: #1]}\else [DCH: #1] \fi}}
%

 %\renewcommand{\ol} [1]{}
 %\renewcommand{\lh} [1]{}
 %\renewcommand{\js} [1]{}
 %\renewcommand{\vh} [1]{}
 % \renewcommand{\dch}[1]{}

\newcommand{\numbersNatural}[0]{\mathbb{N}}
\newcommand{\varss}{\mathbb{X}_s}
\newcommand{\varsi}{\mathbb{X}_i}


\newcommand{\inverse}[1]{{#1}^{-1}}

\newcommand{\defiff}[0]{\stackrel{\text{\tiny def.}}{\Leftrightarrow}}

\newcommand{\col}[0]{\mathcal{C}}
\newcommand{\stcol}[0]{\textsf{col}}
\newcommand{\aut}[0]{A}
\newcommand{\but}[0]{B}
\newcommand{\autof}[1]{\aut_{#1}}
\newcommand{\lassoAutOf}[1]{\autof{#1}^{\text{lasso}}}
\newcommand{\ctype}[0]{\textsf{T}}
\newcommand{\alltypes}[0]{\mathcal{T}}
\newcommand{\stof}[1]{\textsf{st}(#1)}
\newcommand{\autca}[0]{\autof C}
\newcommand{\autaux}[0]{\autof{\mathit{aux}}}

\newcommand{\autass}{\mathsf{Aut}}
% \newcommand{\langAssign}{\mathsf{Lang}}
% \newcommand{\langAssign}{\reg}}
\newcommand{\langAssign}{\constraintsRegulars}
\newcommand{\langAssignOf}[1]{\langAssign(#1)}
\newcommand{\refine}{\mathtt{refine}}
\newcommand{\unify}{\mathtt{unify}}
\newcommand{\noodlify}{\mathtt{noodlify}}
\newcommand{\noodlifyLengths}{\mathtt{noodlifyLen}}
\newcommand{\noodlification}{\textsc{Noodlify}}
\newcommand{\noodle}{\mathsf{N}}
\newcommand{\noodles}{\mathit{Noodles}}
\newcommand{\cond}{\mathit{cond}}
\newcommand{\monadicFormOf}[1]{\mathtt{concatFree}(#1)}
% \newcommand{\monadicFormFormula}{\ensuremath{\psi^{\monadicFormOf{c_\formula}}}\xspace}
\newcommand{\formFormula}{\ensuremath{\psi}\xspace}
% \newcommand{\freshVars}{\mathbb{F}}
\newcommand{\freshVars}{\mathtt{Fresh}}
% \newcommand{\freshVars}{\ensuremath{V}\xspace}
\newcommand{\freshVarsSeqOf}[1]{\ensuremath{\freshVars_{#1}}\xspace}

\newcommand{\variant}[0]{\mathop{\vartriangleleft}}

%Typewriter-like subseteq, from package stix.sty
\makeatletter
\DeclareFontEncoding{LS1}{}{}
\makeatother
\DeclareFontSubstitution{LS1}{stix}{m}{n}
\DeclareSymbolFont{stixletters}{LS1}{stix}{m}{it}
\DeclareSymbolFont{stixoperators}{LS1}{stix}{m}{n}

\DeclareMathSymbol{\othersubseteq}{\mathrel}{stixletters}{"D3}
\DeclareMathSymbol{\otherin}{\mathrel}{stixoperators}{"CB}
\DeclareMathSymbol{\othereq}{\mathrel}{stixoperators}{`=}

% nodes of graph
% \newcommand{\graphnode}[2]{\tikz[baseline,anchor=base]{\node[draw,rounded corners=1mm,fill=black!20,inner sep=0.6mm] {$\vphantom{A_1^2}#1 \subseteq #2$};}}
%\newcommand{\graphnode}[2]{\tikz[baseline,anchor=base]{\node[draw=black!99,rounded corners=0.5mm,fill=black!0,inner sep=0.5mm,text height=2mm,text depth=0.5mm] {$\vphantom{A_1^2}#1 \subseteq #2$};}}
% \newcommand{\graphnode}[2]{ #1 \subseteq #2}
%\newcommand{\graphnode}[2]{ {\mathsf #1} \! \othersubseteq \! {\mathsf #2}}
\newcommand{\graphnodeEq}[2]{{#1} \! \othersubseteq \! {#2}}
\newcommand{\graphnodeFt}[2]{ \transductionArgs{#1}{#2} }
\newcommand{\graphnodeFtInv}[2]{ \transductionArgsInv{#1}{#2} }

\newcommand{\tterm}{t}
\newcommand{\sterm}{s}

\newcommand{\product}{\cap}
\newcommand{\bigproduct}{\bigcap_\varepsilon}
% \newcommand{\bigproduct}{\bigcap_\epsilon}
\newcommand{\reduce}{\mathit{minimise}}
\newcommand{\balance}{\mathtt{balance}}
%\newcommand{\concat}{\circ}
\newcommand{\concat}{\cdot}
\newcommand{\concatof}[1]{\circ(#1)}
\newcommand{\concatxof}[1]{\circ_{#1}}
\newcommand{\concatepsof}[1]{\circ_\varepsilon(#1)}
% \newcommand{\concatepsof}[1]{\circ_\epsilon(#1)}
\newcommand{\concats}{\cdots}

\newcommand{\tightset}{\mathcal T}
\newcommand{\M}{\mathcal M}
% \newcommand{\lang}{\mathcal{L}}

\newcommand{\langOf}[1]{\lang(#1)}
\newcommand{\langOfTick}[1]{\lang'(#1)}
\renewcommand{\prod}{\mathit{Product}}
\newcommand{\lprod}{\mathit{l\text{-}prod}}
\newcommand{\lrprod}{\mathit{lr\text{-}prod}}

\newcommand{\varsn}{\mathsf{vars}}

\newcommand{\formula}{{\varphi}}

\newcommand{\propagate}{\mathtt{propagate}}
\newcommand{\graph}{G}
% \newcommand\constreq{{\mathcal {E}}}
% \newcommand\constrreg{{\mathcal {R}}}
% \newcommand\constrlen{{\Psi}}
% \newcommand\constreq{{\mathscr {E}}}
% \newcommand\constrreg{{\mathscr {R}}}
% \newcommand\constrlen{{\mathscr{L}}}
%\newcommand\constreq{{\mathfrak {E}}}
%\newcommand\constrreg{{\mathfrak {R}}}
%\newcommand\constrlen{{\mathfrak{L}}}

\newcommand\lenSol{\varphi^\ell}
\newcommand\constrEq{{\mathbb{E}}}
\newcommand{\constrFt}{{\mathbb{T}}}
\newcommand\constrReg{{\mathbb{R}}}
\newcommand{\constrreg}{\constrReg}
\newcommand\constrLen{{\mathbb{L}}}
%\newcommand\lenimg{\psi}
% \newcommand\impliedlen{\Psi}
\newcommand\impliedlen{\constrlen}
\newcommand{\constrautass}{\autass_\constr}
\newcommand\constr{\Phi}
\newcommand{\vertices}{V}
\newcommand{\edges}{E}
\newcommand{\vars}{\mathbb X}
% \newcommand{\lenvars}{\mathtt {Len}}
\newcommand{\lenvars}{\mathtt{LVar}}
\newcommand{\monovars}{\mathbb M}
%\newcommand{\sat}{\mathtt{SAT}}
%\newcommand{\unsat}{\mathtt{UNSAT}}
\newcommand{\branches}[0]{\mathit{Branches}}
\newcommand{\lifo}[1]{\langle #1 \rangle}
\newcommand{\pop}{\mathtt{dequeue}}
\newcommand{\push}{\mathtt{enqueue}}

\newcommand{\toolfont}[1]{\textsc{#1}}
\newcommand{\mata}{\toolfont{Mata}\xspace}
\newcommand{\ziiinoodler}{\toolfont{Z3-Noodler}\xspace}
\newcommand{\ziiinoodlernopre}{\toolfont{Z3-Noodler-WI}\xspace}
\newcommand{\ziiinoodlernohomo}{\toolfont{Z3-Noodler-WH}\xspace}
\newcommand{\ziiinoodlerold}{\toolfont{Z3-Noodler} 1.3\xspace}
\newcommand{\toolmodel}[1]{#1$^\M$}
\newcommand{\ziiinoodlermodel}{\toolmodel{\toolfont{Z3-Noodler}}\xspace}
\newcommand{\noodler}{\ziiinoodler}
\newcommand{\cvc}{\toolfont{cvc}\xspace}
\newcommand{\cvcv}{\cvc{}5\xspace}
\newcommand{\cvcvmodel}{\toolmodel{\toolfont{cvc}5}\xspace}
\newcommand{\cvciv}{\cvc{}4\xspace}
\newcommand{\ziii}{\toolfont{Z3}\xspace}
\newcommand{\ziiimodel}{\toolmodel{\toolfont{Z3}}\xspace}
\newcommand{\ziiistriiire}{\toolfont{Z3str3RE}\xspace}
\newcommand{\ziiistriv}{\toolfont{Z3str4}\xspace}
\newcommand{\ziiitrau}{\toolfont{Z3-Trau}\xspace}
\newcommand{\keplertool}[0]{\toolfont{Kepler}$_{\mathtt{22}}$\xspace}
\newcommand{\ostrich}[0]{\toolfont{OSTRICH}\xspace}
\newcommand{\ostrichmodel}{\toolmodel{\toolfont{OSTRICH}}}
\newcommand{\retro}[0]{\toolfont{Retro}\xspace}
\newcommand{\sloth}[0]{\toolfont{Sloth}\xspace}
\newcommand{\jsa}[0]{\toolfont{JSA}\xspace}
\newcommand{\stranger}[0]{\toolfont{Stranger}\xspace}
\newcommand{\trau}[0]{\toolfont{Trau}\xspace}
\newcommand{\norntool}[0]{\toolfont{Norn}\xspace}
\newcommand{\vbs}[0]{\toolfont{VBS}\xspace}
\newcommand{\vbsnoodler}[0]{\toolfont{VBS}$^+$\xspace}

\newcommand{\sumcol}[1]{\textit{#1}}
\newcommand{\benchfont}[1]{\textsf{#1}}
\newcommand{\nornbench}{\benchfont{Norn}\xspace}
\newcommand{\slog}{\benchfont{Slog}\xspace}
\newcommand{\slent}{\benchfont{Slent}\xspace}
\newcommand{\sygusqgen}{\benchfont{Sygus-qgen}\xspace}
\newcommand{\leetcode}{\benchfont{LeetCode}\xspace}
\newcommand{\kaluza}{\benchfont{Kaluza}\xspace}
\newcommand{\woorpje}{\benchfont{Woorpje}\xspace}
\newcommand{\keplerbench}{\benchfont{Kepler}\xspace}
\newcommand{\fullstrint}{\benchfont{FullStrInt}\xspace}
\newcommand{\pyex}{\benchfont{PyEx}\xspace}
\newcommand{\strsmall}{\benchfont{StrSmallRw}\xspace}
\newcommand{\stringfuzz}{\benchfont{StringFuzz}\xspace}
\newcommand{\webapp}{\benchfont{Webapp}\xspace}
\newcommand{\denghang}{\benchfont{Denghang}\xspace}
\newcommand{\transducerplus}{\benchfont{Transducer+}\xspace}
\newcommand{\automatark}{\benchfont{AutomatArk}\xspace}
\newcommand{\redos}{\benchfont{Redos}\xspace}
\newcommand{\omark}{\benchfont{Omark}\xspace}
\newcommand{\pcp}{\benchfont{PCP}\xspace}
\newcommand{\rna}{\benchfont{RNA}\xspace}

\newcommand{\nornbenchshort}{\benchfont{Norn}\xspace}
\newcommand{\slogshort}{\benchfont{Slog}\xspace}
\newcommand{\slentshort}{\benchfont{Slent}\xspace}
\newcommand{\sygusqgenshort}{\benchfont{Syg}\xspace}
\newcommand{\leetcodeshort}{\benchfont{Leet}\xspace}
\newcommand{\kaluzashort}{\benchfont{Kal}\xspace}
\newcommand{\woorpjeshort}{\benchfont{Woo}\xspace}
\newcommand{\keplerbenchshort}{\benchfont{Kep}\xspace}
\newcommand{\fullstrintshort}{\benchfont{StrInt}\xspace}
\newcommand{\pyexshort}{\benchfont{PyEx}\xspace}
\newcommand{\strsmallshort}{\benchfont{StrSm}\xspace}
\newcommand{\stringfuzzshort}{\benchfont{StrFuzz}\xspace}
\newcommand{\webappshort}{\benchfont{Web}\xspace}
\newcommand{\denghangshort}{\benchfont{Den}\xspace}
\newcommand{\transducerplusshort}{\benchfont{Tran+}\xspace}
\newcommand{\automatarkshort}{\benchfont{Aut}\xspace}

\newcommand{\benchcategoryfont}[1]{\textbf{#1}}
\newcommand{\regexbench}{\benchcategoryfont{Regex}\xspace}
\newcommand{\eqbench}{\benchcategoryfont{Equations}\xspace}
\newcommand{\predbench}{\benchcategoryfont{Predicates}\xspace}

\newcommand{\QFStrings}{QF\_Strings\xspace}
\newcommand{\QFS}{\texttt{QF\_S}\xspace}
\newcommand{\QFSLIA}{\texttt{QF\_SLIA}\xspace}
\newcommand{\QFSNIA}{\texttt{QF\_SNIA}\xspace}

%\newcommand{\lass}{\mathsf{la}}
%\newcommand{\constrlass}{\lass}
%\newcommand{\reflass}{\mathsf{la}'}
% \newcommand{\lass}{R}
% \newcommand{\lass}{\constrreg}
\newcommand{\lass}{\langAssign}
\newcommand{\constrlass}{\lass}
\newcommand{\reflass}{\lass'}
\newcommand{\ass}{\nu}
\newcommand{\lf}[1]{\mathtt{Len}(#1)}

\newcommand{\unifnodes}{\mathit{UnifNode}}
\newcommand{\subst}{\sigma}
\newcommand{\substinv}{\subst^\bullet}
\newcommand{\startmark}[1]{\langle_{#1}}
\newcommand{\stopmark}[1]{\rangle_{#1}}
\newcommand{\markedlang}[1]{\startmark{#1}\concat\autass(#1)\concat\stopmark{#1}}
% \newcommand{\dr}{\bullet}
% \newcommand{\dl}{\#}

%\newcommand{\separ}{\sharp}
%\newcommand{\lsepar}{\separ_L}
%\newcommand{\rsepar}{\separ_R}
%\newcommand{\separ}{\mathbb { s}}
%\newcommand{\lsepar}{\mathbb { l}}
%\newcommand{\rsepar}{\mathbb { r}}
%\newcommand{\separ}{\mathbin{\mathbf { s}}}
%\newcommand{\lsepar}{\mathbin{\mathbf { l}}}
%\newcommand{\rsepar}{\mathbin{\mathbf { r}}}
\newcommand{\lsign}{\mathtt{l}}
\newcommand{\rsign}{\mathtt{r}}
\newcommand{\separ}{\pmb {|}}
%\newcommand{\lsepar}{\separ_{\lsign}}
%\newcommand{\rsepar}{\separ_{\rsign}}
%\newcommand{\lsepar}{{\pmb \rfloor}}
%\newcommand{\rsepar}{{\pmb \lfloor}}
% \newcommand{\lsepar}{\fbox{\texttt{L}}}
% \newcommand{\rsepar}{\fbox{\texttt{R}}}
% \newcommand{\lsepar}{\tikz[anchor=base,baseline]{\node[draw,inner sep=0.1mm,minimum height=3.5mm] {\texttt{L}};}}
% \newcommand{\rsepar}{\tikz[anchor=base,baseline]{\node[draw,inner sep=0.1mm,minimum height=3.5mm] {\texttt{R}};}}
% \newcommand{\lsepar}{\tikz[anchor=base,baseline]{\node[inner sep=0.1mm,minimum height=3.5mm,fill=blue!20] {\texttt{L}};}}
% \newcommand{\rsepar}{\tikz[anchor=base,baseline]{\node[inner sep=0.1mm,minimum height=3.5mm,fill=red!20] {\texttt{R}};}}
% \newcommand{\lsepar}{{\pmb \langle}}
% \newcommand{\rsepar}{{\pmb \rangle}}
%\newcommand{\lsepar}{{\rfloor}}
%\newcommand{\rsepar}{{\lfloor}}
\newcommand{\agni}{%
	\begin{tikzpicture}[x=1.4ex, y=1.4ex, scale=0.5, baseline=-.8ex]
		\draw[semithick] (-1,1)  -- (0,1)  -- (0,-1) -- (1,-1);
		\draw[semithick] (-1,-1) -- (-1,0) -- (1,0)  -- (1,1);
	\end{tikzpicture}%
}

% \newcommand{\lsepar}{{\agni}}
%\newcommand{\lsepar}{{\varspadesuit}}
%\newcommand{\lsepar}{{\vardiamondsuit}}
%  \newcommand{\lsepar}{{\varclubsuit}}
%  \newcommand{\rsepar}{{\heartsuit}}
\newcommand{\lsepar}{{\vartriangleleft}}
\newcommand{\rsepar}{{\vartriangleright}}

\newcommand{\lseg}{\mathsf{lseg}}
\newcommand{\rseg}{\mathsf{rseg}}
%\newcommand{\leftterm}[1]{t_{x_{#1}}}
%\newcommand{\rightterm}[1]{t_{y_{#1}}}
%\newcommand{\leftterm}[1]{t^\lsign_{#1}}
%\newcommand{\rightterm}[1]{t^\rsign_{#1}}
\newcommand{\leftterm}[1]{\mathtt s_{#1}}
\newcommand{\rightterm}[1]{\mathtt t_{#1}}
\newcommand{\seg}{\mathsf{seg}}
\newcommand{\shuffle}{\mathbin{\raisebox{\depth}{\rotatebox{270}{$\exists$}}}} %if we don't use stix package

\newcommand{\aore}{a}

\newcommand{\pow}[1]{\mathcal{P}(#1)}
% \newcommand{\Min}[1]{#1^{^{{\hspace{-6mm}{\raisebox{-1pt}{$\scriptscriptstyle{\min}$}}}}}}
\newcommand{\Min}[1]{#1^{\min}}
%\raisebox{distance}[extend-above][extend-below]{text}
\newcommand{\aligneq}{\mathit{Align}}
\newcommand{\aligneqin}{\texttt{in}}
\newcommand{\aligneqout}{\texttt{out}}
\newcommand{\laligneq}{\mathit{l\text{-}align}}
\newcommand{\raligneq}{\mathit{r\text{-}align}}
% \newcommand{\alignsplit}[0]{\textsc{Align-and-Split}\xspace}
\newcommand{\alignsplit}[0]{\textsc{Align\&Split}\xspace}
\newcommand{\stabilization}[0]{\textsc{Stabilization}\xspace}
\newcommand{\convergence}[0]{\textsc{ConstraintConvergence}\xspace}
\newcommand{\chainFreeFragment}{\textsc{Chain-Free}\xspace}

\newcommand{\lnref}[1]{Line~\ref{#1}}
\newcommand{\condref}[1]{(IG\ref{#1})}
\newcommand{\igcondref}[1]{Condition~\condref{#1}}

\newcommand{\inclusionType}{\mathtt{incl}}
\newcommand{\transducerMembershipType}{\mathtt{transmemb}}
\newcommand{\minlangof}[1]{\Min{\lang}(#1)}
\newcommand{\propagatemin}{\mathtt{propagate}_{\mathit{min}}}

% \newcommand{\G}{G}
% \newcommand{\incls}{{\mathbb{I}}}
% \newcommand{\incls}{{\mathbb{V}}}
% \newcommand{\incls}{{\mathsf{Node}}}
\newcommand{\incls}{{\mathsf{N}}}
\newcommand{\constraints}{{\mathbb{C}}}
\newcommand{\constraintPredicates}{{\constraints_p}}
\newcommand{\constraintPredicatesOf}[1]{{\constraints_p(#1)}}
\newcommand{\constraintPredicateTypes}{\constraints_p^T}
\newcommand{\constraintPredicateType}[0]{\omega}
\newcommand{\constraintPredicateTypeOf}[1]{\constraintPredicateType(#1)}
\newcommand{\constraintPredicateTerms}[0]{\tau}
\newcommand{\constraintPredicateTermsOf}[1]{\constraintPredicateTerms(#1)}
\newcommand{\core}{C}
\newcommand{\splitvars}{Z}
%\newcommand{\gnode}{\alpha}
%\newcommand{\gnode}{\graphnode\sterm\tterm}
\newcommand{\gnode}{\iota}
\newcommand{\ruleName}[1]{\textsc{#1}}
\newcommand{\ruleDef}[4]{
{\small
\ruleName{#1}:
\begin{array}{c}
	{#2}
	\\ \hline
	{#3}
\end{array}\
{#4}
}
}
% \newcommand{\constraintGraphWorklist}{\mathsf{Work}}
\newcommand{\constraintGraphWorklist}{\mathsf{WL}}

\newcommand{\infer}[4][]{\ensuremath{#1:\frac{#3}{#2}#4}}
\newcommand{\splinters}{\mathit{R}}
\newcommand{\succof}[2]{#1(#2)}
% \newcommand{\noodlifysplit}{\mathtt{LR\text{-}noodles}}
% \newcommand{\noodlifyrefine}{\mathtt{L\text{-}noodles}}
\newcommand{\noodlifysplit}{\mathtt{LR\text{-}noodlify}}
\newcommand{\noodlifyrefine}{\mathtt{L\text{-}noodlify}}
\newcommand{\noodlifyStable}{\mathtt{ConToSt}}
\newcommand{\noodlifyMonadic}{\mathtt{ConToCF}}
\newcommand{\noodlifyStableFt}{\mathtt{TrToSt}}
\newcommand{\noodlifyMonadicFt}{\mathtt{TrToCF}}
\newcommand{\refineStable}{\textsc{RefineSt}}
\newcommand{\refineMonadic}{\textsc{RefineCF}}
\newcommand{\lconcat}{{::}}

\newcommand{\varsFnName}{\mathtt{Var}}
\newcommand{\varsSeqFnName}{\mathtt{VarSeq}}
\newcommand{\varsOf}[1]{\varsFnName(#1)}
\newcommand{\varsSeqOf}[1]{\varsSeqFnName(#1)}
\newcommand{\varsSeqAt}[2]{\varsSeqFnName(#1)[#2]}
\newcommand{\varsNumIn}[2]{\mathtt{VarNum_{#2}}(#1)}

\newcommand{\tape}{\rho}
\newcommand{\tapeNum}[1]{\tape_{#1}}
% \newcommand{\tapeOf}[2]{{\prescript{#2}{}#1}}
\newcommand{\tapeNumOf}[2]{{\tapeNum{#1}({#2})}}
\newcommand{\varsOfTape}[2]{\varsOf{\tapeNumOf{#2}{#1}}}

\newcommand{\limpl}[0]{\mathrel{\Rightarrow}}
\newcommand{\liff}[0]{\mathrel{\Leftrightarrow}}

\newcommand{\parikh}[0]{\Psi}
\newcommand{\parikhof}[1]{\parikh(#1)}

% disequality symbol
\newcommand{\dsof}[1]{\langle#1\rangle}
\newcommand{\tagmis}[0]{\textbf{\textsf{M}}}
\newcommand{\tagpos}[0]{\textbf{\textsf{P}}}
\newcommand{\taglen}[0]{\textbf{\textsf{L}}}
\newcommand{\tagreg}[0]{\textbf{\textsf{R}}}

% formulae for disequalities
\newcommand{\formdiseqlen}[0]{\varphi_{\mathit{len}}}
\newcommand{\formdiseqpos}[0]{\varphi_{\mathit{pos}}}

% formulae for Parikh image
% \newcommand{\statevarof}[1]{\alpha_{#1}}     % variable for state
% \newcommand{\transvarof}[1]{\beta_{#1}}      % variable for transition
\newcommand{\transvarof}[1]{\numof{#1}}      % variable for transition
\newcommand{\initvarof}[1]{\gamma^I_{#1}}    % variable for initiality of state
\newcommand{\finalvarof}[1]{\gamma^F_{#1}}   % variable for finality of state
\newcommand{\formkirchhoff}[0]{\varphi_{\mathit{Kirch}}}
\newcommand{\forminitstates}[0]{\varphi_{\mathit{Init}}}
\newcommand{\formfinalstates}[0]{\varphi_{\mathit{Fin}}}
\newcommand{\formspan}[0]{\varphi_{\mathit{Span}}}
\newcommand{\formsymb}[0]{\varphi_{\mathit{Symb}}}
\newcommand{\spanningvarof}[1]{\sigma_{#1}}
\newcommand{\misposof}[2]{\lambda^{#2}_{#1}}  % #2-th mismatch for disequality #1

\newcommand{\diseqregsat}[0]{\textsc{DiseqRegSAT}\xspace}
\newcommand{\clNP}[0]{\textsc{NP}}
\newcommand{\clP}[0]{\textsc{PTime}}

% \newcommand{\delim}[0]{\texttt{;}}
\newcommand{\delim}[0]{d}
\newcommand{\lhs}[0]{\mathtt{LHS}}
\newcommand{\rhs}[0]{\mathtt{RHS}}

\newcommand{\dist}[0]{\mathsf{dist}}
\newcommand{\disstr}[0]{\mathsf{disstr}}

\newcommand{\semof}[1]{\llbracket #1 \rrbracket}
%\newcommand{\lang}{\ensuremath{\ell}}
\newcommand{\lang}{L}

\newcommand{\singleoccur}{\mathtt{single}}

\newcommand{\RGBcircle}[1]{\ensuremath{{\color[RGB]{#1}\bullet}}}

\newcommand{\eqs}{\mathcal{\bar E}}
% \newcommand{\eqs}{\overline{\mathcal{E}}}
\newcommand{\reg}{\constraintsRegulars}
\newcommand{\constraintsEquations}{\strpr{Eq}}
\newcommand{\constraintsLengths}{\strpr{Len}}
\newcommand{\constraintsRegulars}{\strpr{Reg}}
\newcommand{\constraintsTransducers}{\strpr{Tr}}
% \newcommand{\solvedeqs}{\strpr{SolEq}}
\newcommand{\solvedeqs}{\strpr{SEq}}
\newcommand{\substEq}{\solvedeqs}
\newcommand{\solvedlia}{\strpr{LE}}
% \newcommand{\constraintsEquations}{\mathcal{E}}
% \newcommand{\constraintsLengths}{\mathcal{L}}
% % \newcommand{\constraintsRegulars}{\reg}}
% \newcommand{\constraintsRegulars}{\mathcal{R}}
% \newcommand{\constraintsTransducers}{\mathcal{T}}
\newcommand{\constraintsLengthsFor}[1]{\constraintsLengths[#1]}

\newcommand{\transducerConstraint}{\mathbb{T}}
\newcommand{\simpleTransducerConstraint}{\transducerConstraint}
\newcommand{\simpleTransducerConstraints}{\constraintsTransducers}
\newcommand{\outputSimpleTransducerConstraints}{\constraintsTransducers^{\text{ob}}}

\newcommand{\simpleTransducerConstraintsEqClass}{\mathbb{E}}
\newcommand{\dependentTransducerConstraintRelation}[0]{\sim_{\simpleTransducerConstraint}}
\newcommand{\dependentTransducerConstraintRelationClosure}[0]{\overline{\dependentTransducerConstraintRelation}}
\newcommand{\dependentTransducerConstraintRelationArgs}[2]{{#1} \dependentTransducerConstraintRelation {#2}}
\newcommand{\dependentTransducerConstraintRelationClosureArgs}[2]{{#1} \dependentTransducerConstraintRelationClosure {#2}}
\newcommand{\dependentTransducerConstraintRelationClosureQuotientSet}{\simpleTransducerConstraints_{/ \dependentTransducerConstraintRelationClosure }}

\newcommand{\triplet}[3]{\langle #1, #2, #3 \rangle}
\newcommand{\ikset}[1]{\left\{#1\right\}^k_{i=1}}
\newcommand{\ikbigl}[0]{\bigl\{}
\newcommand{\ikbigr}[0]{\bigr\}^k_{i=1}}

\newcommand{\code}[0]{\mathsf{code}}

\def\markbaseline{-.28em}   % from spot
\newcommand{\colcircle}[1]{node[left,shape=circle,inner sep=1pt,scale=0.7,fill=orange!60!black,text=white,draw=orange!60!black]  {\sf #1}}
\newcommand{\textcolcircle}[1]{\tikz[baseline=\markbaseline,scale=0.5]{ \draw \colcircle{#1};}}

\newcommand{\regex}{\mathcal{R}}

\newcommand{\smtlib}[0]{SMT-LIB\xspace}

\newcommand{\strpr}[1]{\texttt{#1}\xspace}
\newcommand{\substr}{\strpr{substr}}
\newcommand{\at}{\strpr{at}}
\newcommand{\replace}{\strpr{replace}}
\newcommand{\replaceall}{\strpr{replaceAll}}
\newcommand{\replacere}{\strpr{replace\_re}}
\newcommand{\replacereall}{\strpr{replace\_re\_all}}
\newcommand{\indexof}{\strpr{indexof}}
\newcommand{\contains}{\strpr{contains}}
\newcommand{\notcontains}{\neg\contains}
% \newcommand{\prefix}{\strpr{prefix}}
\newcommand{\prefix}{\strpr{prefixof}}
% \newcommand{\suffix}{\strpr{suffix}}
\newcommand{\suffix}{\strpr{suffixof}}
\newcommand{\isdigit}{\strpr{is\_digit}}
\newcommand{\toint}{\strpr{to\_int}}
\newcommand{\fromint}{\strpr{from\_int}}
\newcommand{\tocode}{\strpr{to\_code}}
\newcommand{\fromcode}{\strpr{from\_code}}
\newcommand{\lenStr}[0]{\strpr{len}}
\newcommand{\lenOfStr}[1]{\lenStr(#1)}
\newcommand{\lenvar}[1]{\lenStr_{#1}}
\newcommand{\lenOf}[1]{|{#1}|}

\newcommand{\Rplus}{\protect\hspace{-.1em}\protect\raisebox{.35ex}{\smaller{\smaller\textbf{+}}}}
\newcommand{\Cpp}{\mbox{C\Rplus\Rplus}\xspace}

% Nielsen transformation
\newcommand{\trim}[0]{\mathsf{trim}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\vecx}{\boldsymbol{x}}
\newcommand{\vecy}{\boldsymbol{y}}
\newcommand{\veca}{\boldsymbol{a}}
\newcommand{\idfl}{\mathit{id}}
\newcommand{\slp}{\mathit{sl}}

% Length-based decision procedure
\newcommand{\begof}[2]{B^{#1}_{#2}}
\newcommand{\lit}[0]{\mathsf{lit}}
\newcommand{\litall}[0]{\mathsf{litall}}
\newcommand{\pos}[0]{\mathsf{pos}}
\newcommand{\comp}[0]{\mathsf{comp}}
\newcommand{\mis}[0]{\mathsf{mis}}
\newcommand{\alignlit}[0]{\mathsf{align}}
\newcommand{\out}[0]{\mathsf{out}}
\newcommand{\excl}[0]{\mathsf{excl}}

% Regexes
\newcommand{\retoaut}[0]{\mathsf{aut}}
\newcommand{\lundef}[0]{\mathsf{undef}}
\newcommand{\sregex}[0]{\mathcal{S}}
\newcommand{\rregex}[0]{\mathcal{R}}

% Procedures
\newcommand{\decproc}[0]{\mathcal{D}}
\newcommand{\unsat}[0]{\mathsf{unsat}}
\newcommand{\sat}[0]{\mathsf{sat}}
\newcommand{\unknown}[0]{\mathsf{unknown}}
\newcommand{\preprocess}[0]{\mathsf{preprocess}}
\newcommand{\init}[0]{\mathsf{init}}
% \newcommand{\computenext}[0]{\mathsf{getSolution}}
\newcommand{\computenext}[0]{\mathsf{nextSolution}}
\newcommand{\getlengths}[0]{\mathsf{getLIA}}
\newcommand{\getmodel}[0]{\mathsf{getModel}}
\newcommand{\liamodel}[0]{\theta}
\newcommand{\issuitable}[0]{\mathsf{isSuitable}}
\newcommand{\bool}[0]{\mathbb{B}}
\newcommand{\boolu}[0]{\mathbb{B}_3}
\newcommand{\lia}[0]{\Phi_{\mathsf{LIA}}}
\newcommand{\precision}[0]{\mathbb{P}}
\newcommand{\precise}[0]{\mathsf{precise}}
\newcommand{\underap}[0]{\mathsf{underapprox}}
\newcommand{\overap}[0]{\mathsf{overapprox}}

\newcommand{\decprocfont}[1]{#1}
\newcommand{\regexproc}[0]{\decprocfont{Regex proc.}}
\newcommand{\nielsenproc}[0]{\decprocfont{Nielsen transf.}}
\newcommand{\lengthproc}[0]{\decprocfont{Length-based}}
\newcommand{\stabproc}[0]{\decprocfont{Stabillization-based}}

\newcommand{\ziiinoodlernonielsen}{\toolfont{Z3-Noodler} without \nielsenproc}
\newcommand{\ziiinoodlernolength}{\toolfont{Z3-Noodler} without \lengthproc}
\newcommand{\ziiinoodlernomemb}{\toolfont{Z3-Noodler} without \regexproc}
\newcommand{\ziiinoodleronlystabilization}[0]{\toolfont{Z3-Noodler} only \stabproc}

% figures
\newcommand{\bx}{{\color{blue}{x}}}
\newcommand{\oy}{{\color{orange}{y}}}
\newcommand{\org}[1]{{\color{orange}{#1}}}

% preliminaries
\newcommand{\varslia}{\mathbb{I}}
\newcommand{\varsLenOf}[1]{\mathbb{I}(#1)}
% \newcommand{\varLen}[1]{\uline{#1}}
\newcommand{\varLen}[1]{\overline{#1}}
% \newcommand{\varLen}[1]{\mathbf{#1}}

% substitute for example environment if we need to use wrapfig
\newcommand{\beginexample}[0]{%
	\medskip\noindent\stepcounter{example}\textit{Example~\theexample}. }

% for literals example
\newcommand{\blu}[1]{{\color{blue}{#1}}}
\newcommand{\gre}[1]{{\color{Green}{#1}}}
\newcommand{\litabo}{\org{ab}}
\newcommand{\litabb}{\blu{ab}}
\newcommand{\litabg}{\gre{ab}}
\newcommand{\litcd}{\org{cd}}

\newcommand{\dontCare}{?}
% \newcommand{\concat}{\cdot}
\newcommand{\eps}{\varepsilon}
% \newcommand{\eps}{\epsilon}
\newcommand{\SigmaEps}{\Sigma_\eps}
\newcommand{\SigmaStar}{\Sigma^*}
\newcommand{\SigmaEpsStar}{\SigmaEps^*}
\newcommand{\SigmaEpsTimes}[1]{(\SigmaEps)^#1}

%\newcommand{\projToSet}[2]{\texttt{project\_to}_{#1}(#2)}
%\newcommand{\projOutSet}[2]{\texttt{project\_out}_{#1}(#2)}
%\newcommand{\projInput}[1]{\texttt{project\_input}(#1)}
%\newcommand{\projOutput}[1]{\texttt{project\_output}(#1)}
%\newcommand{\projTo}[2]{\pi_{#1}(#2)}

\newcommand{\projection}[1]{\pi_{#1}}
% \newcommand{\projTo}[2]{\projection{#1}}
\newcommand{\projToSet}[2]{\projection{#1}(#2)}
\newcommand{\projOut}[1]{\projection{-#1}}
\newcommand{\projOutSet}[2]{\projToSet{-#1}{#2}}
\newcommand{\projInput}[1]{\texttt{project\_input}(#1)}
\newcommand{\projOutput}[1]{\texttt{project\_output}(#1)}
\newcommand{\projTo}[2]{\projection{#1}(#2)}


\newcommand{\apply}[2]{\texttt{apply}(#1, #2)}

\newcommand{\level}[1]{\texttt{lev}(#1)}

\newcommand{\fa}[1]{{#1}}
% \newcommand{\aut}{\mathcal{A}}
% \newcommand{\ft}[#1]{\mathcal{#1}}
\newcommand{\ft}[1]{#1}
\newcommand{\ftPreImg}[1]{\preImg{#1}}
\newcommand{\ftSynchronization}[1]{#1^{\text{sync}}}

\newcommand{\marker}{\triangledown}
% \newcommand{\markerL}{\marker_l}
% \newcommand{\markerR}{\marker_r}
\newcommand{\markerL}{\triangleleft}
\newcommand{\markerR}{\triangleright}
\newcommand{\markers}{D}
\newcommand{\relationPair}[2]{(#1, #2)}
\newcommand{\relationIdPair}[1]{\relationPair{#1}{#1}}
\newcommand{\relationApplyOn}[2]{\relationImg{#1}{#2}}

% \newcommand{\ftBeginMarker}{\ft_{\text{begin}}}
% \newcommand{\ftEndMarker}{\ft_{\text{end}}}

% \newcommand{\ftRegexRelucReplaceAll}{ \ft^\marker_{x^{+}_{\pi \rightarrow y}} }
% \newcommand{\ftRegexRelucReplaceSingle}{ \ft^\marker_{x^{1}_{\pi \rightarrow y}} }
% \newcommand{\ftRegexRelucAll}{ \ft_{x^{+}_{\pi \rightarrow y}} }
% \newcommand{\ftRegexRelucSingle}{ \ft_{x^{1}_{\pi \rightarrow y}} }

% \newcommand{\ftLiteralRelucReplaceAll}{ \ft^\marker_{x^{+}_{z \rightarrow y}} }
% \newcommand{\ftLiteralRelucReplaceSingle}{ \ft^\marker_{x^{1}_{z \rightarrow y}} }
% \newcommand{\ftLiteralRelucAll}{ \ft_{x^{+}_{z \rightarrow y}} }
% \newcommand{\ftLiteralRelucSingle}{ \ft_{x^{1}_{z \rightarrow y}} }

\newcommand{\replacementAll}[3]{ \replacement^{*}_{#2 \rightarrow #3}(#1) }
\newcommand{\replacementSingle}[3]{ \replacement^{1}_{#2 \rightarrow #3}(#1) }
\newcommand{\ftReplaceAll}[4]{ {\ft{#1}}^{*}_{#3 \rightarrow #4}(#2) }
\newcommand{\ftReplaceSingle}[4]{ {\ft{#1}}^{1}_{#3 \rightarrow #4}(#2) }
% \newcommand{\ftConstraintArgs}[3]{{#3} \in \ft{#1}({#2})}
\newcommand{\ftConstraintArgs}[3]{\ft{#1}({#2}, {#3})}
\newcommand{\relConstraintArgs}[3]{{#1}({#2}, {#3})}

% \newcommand{\restrictionSymbol}{\rho}
% \newcommand{\restrictWordFrom}[2]{\restrictionSymbol_{#2}(#1)}
% \newcommand{\restrictLangFrom}[2]{\restrictionSymbol_{#1}(#2)}
\newcommand{\composePipe}{||}
\newcommand{\compose}[2]{{#2} \circ {#1}}
\newcommand{\composeMarked}[3]{{#2} \circ^{#3} {#1}}
\newcommand{\composeOnTapes}[4]{{#2} \circ_{(#3, #4)} {#1}}
\newcommand{\composeOnTapesMarked}[5]{{#2} \circ^{#5}_{(#3, #4)} {#1}}
\newcommand{\syncOnTapes}[4]{{#2} +_{(#3, #4)} {#1}}
\newcommand{\syncOnTapesMarked}[5]{{#2} +^{#5}_{(#3, #4)} {#1}}


\newcommand{\id}[1]{\text{Id}(#1)\xspace}
\newcommand{\ftId}[2]{\ft{#1}_{\id{#2}}\xspace}
\newcommand{\ftIdSigmaStar}[1]{\ft{#1}_{\id{\Sigma^*}}\xspace}

\newcommand{\states}{Q}
\newcommand{\initialStates}{I}
\newcommand{\finalStates}{F}

\newcommand{\post}{\ensuremath{\mathit{post}}}
% \newcommand{\langof}[1]{\lang(#1)}
% \newcommand{\lang}{\mathcal{L}}

% \newcommand{\code}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\ordvector}{\code{OrdVector}\xspace}
\newcommand{\symbolpost}{\code{SymbolPost}\xspace}
\newcommand{\statepost}{\code{StatePost}\xspace}
\newcommand{\pushb}{\code{push\_back}\xspace}
\newcommand{\popb}{\code{pop\_back}\xspace}
\newcommand{\ins}{\code{insert}\xspace}
\newcommand{\erase}{\code{erase}\xspace}
\newcommand{\deltastruct}{\code{Delta}\xspace}
\newcommand{\postvec}{\code{post}\xspace}
\newcommand{\nfaClass}{\code{Nfa}\xspace}

\newcommand{\dfa}{DFA\xspace}
\newcommand{\nfa}{NFA\xspace}
\newcommand{\dfas}{DFAs\xspace}
\newcommand{\nfas}{NFAs\xspace}
\newcommand{\nft}{NFT\xspace}
\newcommand{\nfts}{NFTs\xspace}
\newcommand{\dft}{DFT\xspace}
\newcommand{\dfts}{DFTs\xspace}


% \newcommand{\bdd}{BDD\xspace}
% \newcommand{\bdds}{BDDs\xspace}
% \newcommand{\concatTuple}{\circ}
\newcommand{\transWord}[1]{\bar{{#1}}}
% \newcommand{\relation}{\ast}
\newcommand{\relation}{R}
% \newcommand{\relationPre}{\preImg{#1}[#2]}
% \newcommand{\arityOf}[1]{\mathrm{arity}({#1})}
\newcommand{\arityOf}[1]{\alpha({#1})}
\newcommand{\relationOf}[1]{\relation(#1)}
\newcommand{\relationRational}{\textsc{RL}\xspace}

\newcommand{\preImg}[1]{#1^{-1}}
\newcommand{\img}[1]{#1}
\newcommand{\relationImg}[2]{\img{#1}[#2]}
\newcommand{\relationPreImg}[2]{\preImg{#1}[#2]}
\newcommand{\nop}{\texttt{nop}\xspace}
\newcommand{\subseq}[1]{\texttt{subseq}({#1})\xspace}

\newcommand{\replacement}{
  % \mathcal{S}
  T
  }
% \newcommand{\replacementArgs}[2]{{#2} \in \replacement({#1})}
% \newcommand{\replacementArgsInv}[2]{{#2} \in \replacement^{-1}({#1})}
% \newcommand{\replacementArgsOf}[3]{{#3} \in \ft{#1}({#2})}
% \newcommand{\replacementArgsInvOf}[3]{{#3} \in \ft{#1}^{-1}({#2})}
\newcommand{\replacementArgs}[2]{\replacement({#1}, {#2})}
\newcommand{\replacementArgsInv}[2]{\replacement^{-1}({#1}, {#2})}
\newcommand{\replacementArgsOf}[3]{\ft{#1}({#2}, {#3})}
\newcommand{\replacementArgsInvOf}[3]{\ft{#1}^{-1}({#2}, {#3} )}
\newcommand{\transduction}{
  % \mathcal{T}
  T
}
% \newcommand{\transductionArgs}[2]{\langOf{{#2}} \in \transduction(\langOf{{#1}})}
% \newcommand{\transductionArgsInv}[2]{\langOf{{#2}} \in \transduction^{-1}(\langOf{{#1}})}
% \newcommand{\transductionArgs}[2]{\transduction(\langOf{{#1}}, \langOf{{#2}})}
% \newcommand{\transductionArgsInv}[2]{\preImg{\transduction}(\langOf{{#1}}, \langOf{{#2}})}
% \newcommand{\transductionArgsOf}[3]{{#1}(\langOf{{#1}}, \langOf{{#2}})}
% \newcommand{\transductionArgsInvOf}[3]{\preImg{{#1}}(\langOf{{#1}}, \langOf{{#2}})}
\newcommand{\transductionArgs}[2]{\transduction({#1}, {#2})}
\newcommand{\transductionArgsInv}[2]{\preImg{\transduction}({#1}, {#2})}
\newcommand{\transductionArgsOf}[3]{{#1}({#2}, {#3})}
\newcommand{\transductionArgsInvOf}[3]{\preImg{{#1}}({#1}, {#2})}

\newcommand{\equationArgs}[2]{#1 = #2}
\newcommand{\equals}{\approx}
\newcommand{\notequals}{\not\approx}
\newcommand{\equationNodeArgs}[2]{#1 \equals #2}
\newcommand{\disequationNodeArgs}[2]{#1 \notequals #2}
\newcommand{\equationArgsInv}[2]{#1 = #2}
\newcommand{\inclusionArgs}[2]{\langOf{#1} \subseteq \langOf{#2}}
\newcommand{\inclusionArgsInv}[2]{\langOf{#1} \subseteq \langOf{#2}}


\newcommand{\toolname}[1]{\textsc{#1}\xspace}
\newcommand{\automatajar}{\toolname{AutomataLib}}
\newcommand{\awali}{\toolname{Awali}}

\newcommand{\owl}{\toolname{Owl}}
\newcommand{\mosel}{\toolname{Mosel}}
\newcommand{\spot}{\toolname{Spot}}
\newcommand{\lash}{\toolname{Lash}}
\newcommand{\mona}{\toolname{Mona}}
% \newcommand{\mata}{\toolname{Mata}}
\newcommand{\matasim}{\toolname{Mata-Sim}}
\newcommand{\enfa}{\toolname{eNfa}}
% \newcommand{\noodler}{\toolname{Z3-Noodler}}
%\newcommand{\cpp}{{{C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\tiny\bf ++}}}\xspace}
\newcommand{\cpp}{C++\xspace}
\newcommand{\csharp}{
	{\settoheight{\dimen0}{C}C\kern-.05em \resizebox{!}{\dimen0}{\raisebox{\depth}{\#}}}\xspace}
\newcommand{\vata}{\toolname{Vata}}
\newcommand{\brics}{\toolname{Brics}}
\newcommand{\automatanet}{\toolname{Automata.net}}
\newcommand{\automatapy}{\toolname{Automata.py}}
\newcommand{\fado}{\toolname{FAdo}}
% \newcommand{\noodler}{\textsc{Tool}\xspace}
% \newcommand{\cvc}{\textsc{cvc}\xspace}
% \newcommand{\cvcv}{\cvc{}5\xspace}
% \newcommand{\cvciv}{\cvc{}4\xspace}
% \newcommand{\ziii}{\textsc{Z3}\xspace}
% \newcommand{\ziiistriiire}{\textsc{Z3str3RE}\xspace}
% \newcommand{\ziiistriv}{\textsc{Z3str4}\xspace}
% \newcommand{\ziiitrau}{\textsc{Z3-Trau}\xspace}
\newcommand{\kepler}[0]{\texttt{Kepler}$_{\mathtt{22}}$\xspace}
% \newcommand{\ostrich}[0]{\textsc{OSTRICH}\xspace}
% \newcommand{\retro}[0]{\textsc{Retro}\xspace}
% \newcommand{\sloth}[0]{\textsc{Sloth}\xspace}
% \newcommand{\jsa}[0]{\textsc{JSA}\xspace}
% \newcommand{\stranger}[0]{\textsc{Stranger}\xspace}
% \newcommand{\trau}[0]{\textsc{Trau}\xspace}
\newcommand{\norn}[0]{\textsc{Norn}\xspace}
% \newcommand{\slog}{\textsc{Slog}\xspace}
% \newcommand{\slent}{\textsc{Slent}\xspace}
% \newcommand{\sygusqgen}{\textsc{Sygus-Qgen}\xspace}
% \newcommand{\leetcode}{\textsc{Leetcode}\xspace}
% \newcommand{\kaluza}{\textsc{Kaluza}\xspace}
\newcommand{\kudzu}{\textsc{Kudzu}\xspace}
% \newcommand{\woorpje}{\textsc{Woorpje}\xspace}
% \newcommand{\keplerbench}{\textsc{Kepler}\xspace}
% \newcommand{\fullstrint}{\textsc{Full-str-int}\xspace}
% \newcommand{\pyex}{\textsc{Pyex}\xspace}
% \newcommand{\strsmall}{\textsc{Str-small-rw}\xspace}
% \newcommand{\regex}{\textsc{Regex}\xspace}

\newcommand{\reverse}[1]{\text{rev(}#1\text{)}\xspace}

% \newcommand{\lindex}{\leftindex^{#1}_{#2} {#3}$
\newcommand{\unionRelation}[2]{{#1} \cup {#2}}
\newcommand{\intersectionRelation}[2]{{#1} \cap {#2}}
\newcommand{\intersectionEpsPresSymb}{\mathrlap{+}\cap}
\newcommand{\intersectionEpsPres}[4]{\prescript{#1}{#2}\intersectionEpsPresSymb^{#3}_{#4}}
\newcommand{\synchronizedProductSymbol}{\ensuremath{\Cap}}
\newcommand{\synchronizedProduct}[1]{\ensuremath{\synchronizedProductSymbol^{#1}}}
\newcommand{\synchronizedProductTapes}[2]{\prescript{#1}{}\synchronizedProductSymbol^{#2}}


\newcommand{\powersetOf}[1]{\mathcal{P}(#1)}
\newcommand{\regLangConcat}[1]{\reg(#1)}
\newcommand{\regLangConcatPresMark}[2]{\reg^{#2}(#1)}

\newcommand{\interval}[2]{[{#1}..{#2}]}

% \newcommand{\ftTransSymb}[2]{\begin{bsmallmatrix}{#1} & {#2}\end{bsmallmatrix}}
\newcommand{\ftTransSymb}[2]{({#1}, {#2})}

\newcommand{\dependentVarsRelation}[0]{\mathcal{\sim}}
\newcommand{\dependentVarsRelationClosure}[0]{\overline{\dependentVarsRelation}}
\newcommand{\dependentVarsRelationArgs}[2]{{#1} \dependentVarsRelation {#2}}
\newcommand{\dependentVarsRelationClosureArgs}[2]{{#1} \dependentVarsRelationClosure {#2}}

\newcommand{\nearzero}{$\sim$0\xspace}
\newcommand{\br}[1]{\textbf{#1}}

%% constraint graph
\newcommand{\constrsys}{
  % \mathcal{C}
  \varphi
  }
\newcommand{\transs}{
  % \mathcal{S}
  T
  }
\newcommand{\transeq}{\trans^=}
\newcommand{\dual}[1]{\mathtt{dual}(#1)}
\newcommand{\incltr}{{\in}}
\newcommand{\nodes}{\mathtt{nodes}}

\newcommand{\rules}{\texttt{rules}}

\newcommand{\ruleStable}{\ruleName{LenImage}}
\newcommand{\ruleStableC}{\ruleName{Stable}_\constrconv}
\newcommand{\ruleSkip}{\ruleName{Skip}}
\newcommand{\ruleRefine}{\ruleName{Refine}}
\newcommand{\ruleLangInter}{\ruleName{LangInter}}
\newcommand{\ruleCombineNonLength}{\ruleName{CombNL}}
\newcommand{\ruleAlignSplit}{\refineStable}
\newcommand{\ruleAlignSplitW}{\ruleAlignSplit}
\newcommand{\ruleAlignSplitLen}{\refineMonadic}
\newcommand{\ruleLSubs}{\ruleName{RSubst}}
\newcommand{\ruleLLSubs}{\ruleName{LSubst}}
\newcommand{\ruleRemoveLenSat}{\ruleName{RemLenSat}}
\newcommand{\rulereducetrans}{\ruleName{RedTrans}}
\newcommand{\rulehomtrans}{\ruleName{HomTrans}}
% \newcommand{\frontier}[0]{\mathsf{Work}}
% \newcommand{\frontier}[0]{\mathsf{WL}}
\newcommand{\frontier}[0]{\mathsf{F}}
\newcommand{\graphnode}[2]{\!\tikz[baseline,anchor=base]{\node[rounded corners=1mm,inner sep=0.6mm,text height=2mm,text depth=0.5mm] {$\vphantom{A_1^2} \mathsf{#1} \! \othersubseteq \! \mathsf{#2}$};}\!}
\newcommand{\gn}{\graphnode}
\newcommand{\shrinkit}{\hspace{-1.8mm}}
\newcommand{\gnst}{\gn{\sterm}{\tterm}}
\newcommand{\gnts}{\gn{\tterm}{\sterm}}
\newcommand{\constrlen}{{\mathcal {L}}}
\newcommand{\stable}{\varphi}
\newcommand{\stablelen}{\stable_{\mathsf{len}}}

\newcommand{\proplen}{\mathtt{PropLen}}
\newcommand{\proplenfw}{\mathtt{LenFw}}
\newcommand{\proplenbw}{\mathtt{LenBw}}
\newcommand{\dep}{\mathtt{dep}}
\newcommand{\refinable}{\mathtt{refinable}}
\newcommand{\refinablecf}{\mathtt{refCF}}
\newcommand{\refinablest}{\mathtt{refSt}}
\newcommand{\uniform}{\mathtt{uniform}}
\newcommand{\mergelass}{\mathtt{merge}}

\input{macromove.tex}
% \newcommand{\move}[3]{{#1} \xrightarrow{{#2}} {#3}}
% \newcommand{\move}[3]{{#1} \xrightarrow{{#2}} {#3}}
% \newcommand{\ftTransition}[3]{{#1} \xrightarrow{{#2}} {#3}}
\newcommand{\ftTransition}[3]{\move{#1}{#2}{#3}}
\newcommand{\ftTransitionTuple}[3]{({#1}, {#2}, {#3})}
% \newcommand{\nfaTransition}[3]{{#1} \xrightarrow{{#2}} {#3}}
\newcommand{\nfaTransition}[3]{\move{#1}{#2}{#3}}
\newcommand{\nfaTransitionTuple}[3]{({#1}, {#2}, {#3})}

%\newcommand{\lenimg}[1]{\psi_{\lenStr}(#1)}
\newcommand{\lenimg}[1]{\mathsf{LenImg}(#1)}
% \newcommand{\lenimgproj}[2]{\lenStr_{#2}(#1)}
\newcommand{\ftT}{\ft{T}}

\newcommand{\noodlificationNft}{\ensuremath{\ft{T}^{M}_{+}}\xspace}
\newcommand{\noodlificationNfa}{\ensuremath{\fa{A}^{M}_{+}}\xspace}
\newcommand{\noodlificationNftLang}{\ensuremath{\ft{T}_{+}}\xspace}
\newcommand{\noodlificationNfaLang}{\ensuremath{\fa{A}_{+}}\xspace}

\newcommand{\inputtrans}{\mathcal{T}}
\newcommand{\chfreestrict}{directly chain-free\xspace}

\newcommand{\dch}[1]{\todo[linecolor=orange,backgroundcolor=orange!25,bordercolor=orange]{DCH: #1}}
\newcommand{\vh}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red]{VH: #1}}
\newcommand{\lh}[1]{\todo[linecolor=magenta,backgroundcolor=magenta!25,bordercolor=magenta]{LH: #1}}
\newcommand{\js}[1]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green]{JS: #1}}

\newcommand{\eqtostable}{\mathtt{EqToSt}}
\newcommand{\eqtomonadic}{\mathtt{EqToCF}}
\newcommand{\formulaToStableMonadic}{\texttt{formulaToStCF}\xspace}

\newcommand{\cubepart}[2]{#2_{#1}}
\newcommand{\ftype}[1]{\texttt{#1}}
\newcommand{\Eq}{\ftype{Eq}}
\newcommand{\Tr}{\ftype{Tr}}
\newcommand{\Reg}{\ftype{Reg}}
\newcommand{\Len}{\ftype{Len}}
\newcommand{\EqTr}{\ftype{EqTr}}
\newcommand{\Str}{\ftype{Str}}
\newcommand{\Eqof}[1]{\cubepart{#1}{\Eq}}
\newcommand{\Trof}[1]{\cubepart{#1}{\Tr}}
\newcommand{\Regof}[1]{\cubepart{#1}{\Reg}}
\newcommand{\Lenof}[1]{\cubepart{#1}{\Len}}
\newcommand{\EqTrof}[1]{\cubepart{#1}{\EqTr}}
\newcommand{\Strof}[1]{\cubepart{#1}{\Str}}
\newcommand{\cube}{\varphi}

\newcommand\stablec{\mathtt{St}}
\newcommand\solvedc{\mathtt{CF}}
\newcommand\stablecOf[1]{\stablec}
\newcommand\solvedcOf[1]{\solvedc}
\newcommand\solvedcReg{\Regof{\cube}^\solvedc}
\newcommand\lenc{\varphi_{Len}}
\newcommand\sharedv{V_{\mathtt{shared}}}
\newcommand\varsof\varsOf
\newcommand{\regc}{\varphi_{Reg}}

\newcommand{\concatenationFree}{concatenation-free\xspace}
\newcommand{\ConcatenationFree}{Concatenation-free\xspace}

\newcommand{\stablef}{\stablec}
\newcommand{\regf}{\varphi_{Reg}}
\newcommand{\lenf}{\lenc}

\newcommand{\VSpaceScale}{0}

\newcommand{\scaledvspace}[1]{%
  \ifdim\VSpaceScale pt=0pt
    % do nothing
  \else
    \vspace{\VSpaceScale\dimexpr#1\relax}%
  \fi
}

